Reconciling the magnetic field in central disc galaxies with the dynamical mass using the cosmological simulations

The Universe is pervaded by magnetic fields in different scales, although for simplicity, they are ignored in most cosmological simulations. In this paper, we use the TNG50, which is a large cosmological galaxy formation simulation that incorporates magnetic fields with an unprecedented resolution. We study the correlation of the magnetic field with various galaxy properties such as the total, stellar and gaseous mass, circular velocity, size and star formation rate. We find a linear correlation between the average magnetic field pervading the disc of galaxies in relative isolation and their circular velocities. In addition we observed that in this sample the average magnetic field in the disc is correlated with the total mass as $\overline{B}\sim M_{\mathrm{tot,\,R_{\star}}}^{0.2}$. We also find that the massive galaxies with active wind-driven black hole feedback, do not follow this trend, as their magnetic field is substantially affected by this feedback mode in the TNG50 simulation. We show that the correlation of the magnetic field with the star formation rate is a little weaker than the circular velocity. Moreover, we compare the magnetic field components of the above sample with a compiled observational sample of non-cluster non-interacting nearby galaxies. Similar to the observation, we find a coupling between the ordered magnetic field and the circular velocity of the flat part of the rotation curve in the simulation, although contrary to the observation, the ordered component is dominant in the simulation.

==> table_TNG_vs_T16.tex <==
\begin{table*}
	\centering
		\caption{Correlation of the magnetic field ($\bcgd$ or $\btot$ in the TNG50 and $\bord$ in the \taba samples) with $\vre$, $\re$ and $\Omegare$. In \taba samples, EQ denotes to the equipartition assumption whereas CR to the $\Ncr\sim\rm{SFR}$ approximation. Moreover, 22 at the end means sample in which irregular galaxies are not considered.}
		\label{tab:TNG_vs_T16}
		\begin{tabular}{ccccccccccc}
			\hline
			%$ $ & $ $ &\multicolumn{2}{c}{$\kappa$} &\multicolumn{2}{c}{$n$} &\multicolumn{1}{c}{$A$}\\ 
			Sample & Property & $\dfrac{\Riso>}{\rm{(Mpc)}}$ & $\Pearson$ & $\Spearman$ & $a$ & Sample & $\dfrac{\Riso>}{\rm{(Mpc)}}$ & $\Pearson$ & $\Spearman$ & $a$ \\
			\hline
%% TNG ========================================================================
			TNG50,\,$\bord$      & $\vrot$       & 1 & 0.46  & 0.43  & 0.95  & TNG50,\,$\bordth$ & 1 & 0.83 & 0.83 & 1.95 \\
			..                   & $\re$         & 1 & -0.09 & -0.09 & -0.10 & .. & 1 & 0.62 & 0.62 & 0.76 \\
			..                   & $\Omegare$    & 1 & 0.41  & 0.35  & 0.53  & .. & 1 & -0.24 & -0.28 & -0.36 \\
			                     \\
			..                   & $\vrot$       & 2 & 0.63 & 0.57 & 1.34 & .. & 2 & 0.90 & 0.88 & 2.37 \\
			..                   & $\re$         & 2 & 0.18 & 0.17 & 0.20 & .. & 2& 0.70 & 0.70 & 0.96 \\
			..                   & $\Omegare$    & 2 & 0.20 & 0.18 & 0.30 & .. & 2 & -0.32 & -0.34 & -0.60 \\
			                     \\
			TNG50,\,$\bturb$     & $\vrot$       & 1 & 0.39  & 0.33  & 0.79  & TNG50,\,$\bturbth$ & 1 & 0.90 & 0.89 & 1.76 \\
			..                   & $\re$         & 1 & -0.36 & -0.34 & -0.37 & .. & 1 & 0.54 & 0.55 & 0.55 \\
			..                   & $\Omegare$    & 1 & 0.69  & 0.63  & 0.88  & .. & 1 & -0.10 & -0.18 & -0.12 \\
			                     \\
			..                   & $\vrot$       & 2 & 0.41  & 0.30  & 0.70  & .. & 2 & 0.93 & 0.92 & 1.89 \\	
			..                   & $\re$         & 2 & -0.20 & -0.22 & -0.18 & .. & 2 & 0.70 & 0.74 & 0.74 \\		
			..                   & $\Omegare$    & 2 & 0.57  & 0.54  & 0.68  & .. & 2 & -0.29 & -0.37 & -0.42 \\
			                     \\
			TNG50,\,$\btot$      & $\vrot$       & 1 & 0.51  & 0.47  & 0.94  & TNG50,\,$\btotth$ & 1 & 0.88 & 0.88 & 1.93 \\
			..                   & $\re$         & 1 & -0.19 & -0.18 & -0.19 & .. & 1 & 0.62 & 0.62 & 0.71 \\
			..                   & $\Omegare$    & 1 & 0.56  & 0.50  & 0.66  & .. & 1 & -0.21 & -0.25 & -0.29 \\
			                     \\
			..                   & $\vrot$       & 2 & 0.65 & 0.55 & 1.18 & .. & 2 & 0.93 & 0.91 & 2.28 \\	
			..                   & $\re$         & 2 & 0.08 & 0.06 & 0.08 & .. & 2 & 0.71 & 0.71 & 0.90 \\
			..                   & $\Omegare$    & 2 & 0.34 & 0.32 & 0.45 & .. & 2 & -0.31 & -0.35 & -0.54 \\
								 \\
		TNG50,\,$\bord/\bturb$	 & $\vrot$       & 1 & 0.08 & 0.12 & 0.16     & TNG50,\,$\bordth/\bturbth$ & 1 & 0.13 & 0.15 & 0.20 \\
			..                   & $\re$         & 1 & 0.27 & 0.25 & 0.27     & .. & 1 & 0.26 & 0.27 & 0.21 \\
			..                   & $\Omegare$    & 1 & -0.28 & -0.24 & -0.34  & .. & 1 & -0.24 & -0.23 & -0.24 \\
								 \\
			..	 				 & $\vrot$       & 2 & 0.34 & 0.35 & 0.65     & .. & 2 & 0.33 & 0.32 & 0.48 \\
			..                   & $\re$         & 2 & 0.38 & 0.35 & 0.38     & .. & 2 & 0.30 & 0.29 & 0.22 \\
			..                   & $\Omegare$    & 2 & -0.28 & -0.24 & -0.38  & .. & 2 & -0.17 & -0.18 & -0.18 \\
%% T16 ========================================================================
			                     &               &   & & & \\			                     
			T16,\,$\bord$		 & $\vrot$       & - & 0.92  & 0.73  & 1.54  & T16\_22,\,$\bord$ & - & 0.74 & 0.56 & 1.23 \\
			..                   & $\re$         & - & 0.82  & 0.65  & 0.77  & .. & - & 0.53 & 0.43 & 0.50 \\
		    ..                   & $\Omegare$    & - & -0.55 & -0.40 & -0.96 & .. & - & -0.16 & -0.11 & -0.22 \\
			                     &               &   & & & \\
			T16,\,$\bturb$		 & $\vrot$       & - &  0.83  & 0.68  & 1.17  & T16\_22,\,$\bturb$ & - & 0.56 & 0.48 & 0.98 \\
			..                   & $\re$         & - &  0.73  & 0.59  & 0.58  & .. & - & 0.36 & 0.32 & 0.36 \\
			..                   & $\Omegare$    & - &  -0.49 & -0.37 & -0.71 & .. & - & -0.06 & -0.05 & -0.08 \\
			&               &   & & & \\
			T16,\,$\btot$		 & $\vrot$       & - &  0.87  & 0.71  & 1.22  & T16\_22,\,$\btot$ & - & 0.63 & 0.53 & 1.04 \\
			..                   & $\re$         & - &  0.77  & 0.61  & 0.61  & .. & - & 0.41 & 0.36 & 0.39 \\
			..                   & $\Omegare$    & - &  -0.51 & -0.37 & -0.75 & .. & - & -0.08 & -0.06 & -0.11 \\
								\\
	T16,\,$\bord/\bturb$		 & $\vrot$       & - & 0.49 & 0.37 & 0.37  & T16\_22,\,$\bord/\bturb$ & - & 0.21 & 0.18 & 0.25 \\
			..                   & $\re$         & - &  0.45 & 0.38 & 0.19  & .. & - & 0.21 & 0.18 & 0.15 \\
			..                   & $\Omegare$    & - &  -0.32 & -0.28 & -0.25 & .. & - & -0.14 & -0.10 & -0.13 \\
%			&               &   & & & \\
%		    T16EQ22 			 & $\vrot$        & - & 0.74  & 0.56 & 1.23\\	
%			..                   & $\re$         & - & 0.53  & 0.43 & 0.50\\
%			..                   & $\Omegare$    & - & -0.16 &-0.11 & -0.22\\
%			                     &               &   & & & \\
%			T16CR 				 & $\vre$        & - & 0.76  & 0.66 & 0.90 \\
%			..                   & $\re$         & - & 0.72  & 0.63 & 0.48 \\
%			..                   & $\Omegare$    & - & -0.54 & -0.47 & -0.65\\
%			                     &               &   & & & \\
%			T16CR22 			 & $\vre$        & - & 0.48  & 0.44 & 0.78\\	
%			..                   & $\re$         & - & 0.44  & 0.40 & 0.41\\
%			..                   & $\Omegare$    & - & -0.24 &-0.23 & -0.32\\			
			\hline
		\end{tabular}
\end{table*}

